Rotational cmc surfaces in terms of Jacobi elliptic functions

We give a classification of rotational cmc surfaces in non-Euclidean space forms in terms of explicit parametrizations using Jacobi elliptic functions. Our method hinges on a Lie sphere geometric description of rotational linear Weingarten surfaces and can thus be applied to a more general class of surfaces. As another application of this framework, we give explicit parametrizations of a class of rotational constant harmonic mean curvature surfaces in hyperbolic space. In doing so, we close the last gaps in the classification of all channel linear Weingarten surfaces in space forms, started in Hertrich-Jeromin et all (2023).

==> Preamble/Packages.tex <==
\usepackage{ifdraft}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amsfonts,amssymb,amsmath,amsthm}
\usepackage{paralist}
\usepackage{verbatim}
\usepackage{etoolbox}
\usepackage{pgfplots}
\pgfplotsset{compat=1.16}

\usepackage[%
  backgroundcolor=newred!30,
  textcolor=newred,
  linecolor=newred,
  bordercolor=newred,
  colorinlistoftodos,
  obeyDraft
]{todonotes}

\usepackage[%
    giveninits=true,% 
    backend=biber,
    style=numeric,
    %refsection=section,
    isbn=false,
    doi=false,
    maxbibnames = 99]{biblatex}
\bibliography{Preamble/literature} %Import the bibliography file
\usepackage{csquotes}
%\renewcommand*{\bibfont}{\footnotesize}

\usepackage{varioref}
\RequirePackage{doi}
\usepackage{hyperref}
\usepackage{cleveref}

\ifdraft{
\usepackage[top=2cm, bottom=2cm, left=1cm, right=4cm, marginparwidth=3cm]{geometry}
\usepackage{showlabels}
}{
\usepackage[top=2cm, bottom=2cm, left=2cm, right=2cm]{geometry}
}
